Propagation Modeling for Physically Large Arrays: Measurements and Multipath Component Visibility

This paper deals with propagation and channel modeling for physically large arrays. The focus lies on acquiring a spatially consistent model, which is essential, especially for positioning and sensing applications. Ultra-wideband, synthetic array measurement data have been acquired with large positioning devices to support this research. We present a modified multipath channel model that accounts for a varying visibility of multipath components along a large array. Based on a geometric model of the measurement environment, we analyze the visibility of specular components. We show that, depending on the size of the reflecting surface, geometric visibility and amplitude estimates obtained with a super-resolution channel estimation algorithm show a strong correspondence. Furthermore, we highlight the capabilities of the developed synthetic array measurement system.

==> figures/results/model_visibility/portal2_pos1_4x4/VA2_window_path_91_model_vis_img/VA2_window_path_91_model_vis_img.tex <==
%!TEX root = ../../../../../../main_d12.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.926\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=28.5,
%xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=18.5,
%ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
%title style={font=\bfseries},
%title={},
xmajorgrids,
ymajorgrids,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
 unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
%colorbar horizontal,
colorbar sampled,
colorbar style={samples=3,at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=6mm,width=1.5mm,ytick={0.25,0.75},yticklabels={not visible,visible},xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xtick distance={1}},%,point meta min=0,point meta max=1}
%colorbar style={samples=3,at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=2mm,width=0.5\figurewidth,xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xlabel=est. amp. in dB,xtick distance={1}},%,point meta min=0,point meta max=1}
%colorbar,
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={geom. vis.}}
]
%from matlab: parula(2)
%0.2422    0.1504    0.6603
%0.9769    0.9839    0.0805
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA2_window_path_91_model_vis_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/model_visibility/portal2_pos1_4x4/VA4_window-doorwall_path_90_23_model_vis_img/VA4_window-doorwall_path_90_23_model_vis_img.tex <==
%!TEX root = ../../../../../../2023_EUCNC.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.926\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=28.5,
%xlabel style={font=\color{white!15!black}},
xlabel={hor. idx.},%{subarray index hor.},
ymin=0.5,
ymax=18.5,
%ylabel style={font=\color{white!15!black}},
ylabel={vert. idx.},%{subarray index vert.},
axis background/.style={fill=white},
%title style={font=\bfseries},
%title={90 23},
xmajorgrids,
ymajorgrids,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
 unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
%colorbar horizontal,
%colorbar sampled,
%colorbar style={samples=3,at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=6mm,width=1.5mm,ytick={0.25,0.75},yticklabels={not visible,visible},xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xtick distance={1}},%,point meta min=0,point meta max=1}
ylabel style={yshift=-1.5mm},
xlabel style={yshift=1.5mm},
%colorbar,
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={geom. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA4_window-doorwall_path_90_23_model_vis_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/VA1_MPC_visibility_img/VA1_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.933\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=28.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=18.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA1_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/VA2_MPC_amplitude_PL-comp_img/VA2_MPC_amplitude_PL-comp_img.tex <==
%!TEX root = ../../../../../../../main_d12.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.926\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-55.0396902656945,
point meta max=-45.0396902656945,
axis on top,
xmin=0.5,
xmax=28.5,
%xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=18.5,
%ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
colorbar horizontal,
colorbar style={at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=1.5mm,width=0.5\figurewidth,xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xlabel=est. amp. in dB,xtick distance={4}}
%colorbar style={at={(1.02,1)},xticklabel pos=right,anchor=north west,major tick length=1mm,width=2mm,height=0.6\figureheight,yticklabel style={rotate=0,font=\footnotesize,xshift=0mm},ylabel=est. amp. in dB}
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA2_MPC_amplitude_PL-comp_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/VA2_MPC_visibility_img/VA2_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.933\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=28.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=18.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA2_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/VA3_MPC_amplitude_PL-comp_img/VA3_MPC_amplitude_PL-comp_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.933\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-55.2355126055864,
point meta max=-45.2355126055864,
axis on top,
xmin=0.5,
xmax=28.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=18.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA3_MPC_amplitude_PL-comp_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/VA3_MPC_visibility_img/VA3_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.933\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=28.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=18.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA3_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/VA4_MPC_visibility_img/VA4_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.933\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=28.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=18.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA4_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/VA5_MPC_visibility_img/VA5_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.933\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=28.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=18.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA5_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/VA6_MPC_amplitude_PL-comp_img/VA6_MPC_amplitude_PL-comp_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.933\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-62.6275180111235,
point meta max=-52.6275180111235,
axis on top,
xmin=0.5,
xmax=28.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=18.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA6_MPC_amplitude_PL-comp_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/VA6_MPC_visibility_img/VA6_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.933\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=28.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=18.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA6_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/VA7_MPC_amplitude_PL-comp_img/VA7_MPC_amplitude_PL-comp_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.933\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-68.5155237269884,
point meta max=-58.5155237269884,
axis on top,
xmin=0.5,
xmax=28.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=18.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA7_MPC_amplitude_PL-comp_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/VA7_MPC_visibility_img/VA7_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.933\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=28.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=18.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA7_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/VA8_MPC_amplitude_PL-comp_img/VA8_MPC_amplitude_PL-comp_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.933\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-47.8627253650303,
point meta max=-37.8627253650303,
axis on top,
xmin=0.5,
xmax=28.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=18.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA8_MPC_amplitude_PL-comp_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/VA8_MPC_visibility_img/VA8_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.933\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=28.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=18.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=28.5, ymin=0.5, ymax=18.5] {\datapath/VA8_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/subarray_14/angle_spectrum_residual_subarray_14/angle_spectrum_residual_subarray_14.tex <==
%!TEX root = ../../../../../../../../2023_EUCNC.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.852\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-30,
point meta max=0,
axis on top,
x dir=reverse,
xmin=-1.01123595505618,
xmax=181.011235955056,
xtick={  0,  45,  90, 135, 180},
%xlabel style={font=\color{white!15!black}},
xlabel={az. in deg},
y dir=reverse,
ymin=-1.52542372881356,
ymax=181.525423728814,
ytick={  0,  45,  90, 135, 180},
%ylabel style={font=\color{white!15!black}},
ylabel={el. in deg},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(1,1,1); rgb(255pt)=(0,0,0)},
%colorbar horizontal,
%colorbar style={at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=1.5mm,width=0.6\figurewidth,xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xlabel={ang.-spect. in dB},xtick distance={10}},
colorbar,
colorbar style={at={(1.02,0)},xticklabel pos=right,anchor=south west,major tick length=1mm,width=1.5mm,height=\figureheight,yticklabel style={rotate=0,font=\footnotesize,xshift=-0.5mm},ylabel={ang.-spect. in dB},ylabel style={yshift=2mm},ytick distance={10}},
ylabel style={yshift=-2mm},
xlabel style={yshift=1.5mm},
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={res. angle spectrum}}
]
\addplot [forget plot] graphics [xmin=-1.01123595505618, xmax=181.011235955056, ymin=-1.52542372881356, ymax=181.525423728814] {\datapath/angle_spectrum_residual_subarray_14-1.png};
\addplot[only marks, mark=+, mark options={}, mark size=1.5811pt, draw=red] table[]{\datapath/angle_spectrum_residual_subarray_14-1.tsv};
\addlegendentry{data1}

\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:99.775,90.968) {1};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:28.093,90.613) {2};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:64.019,90.305) {3};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:161.288,90.2) {4};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:155.514,90.293) {5};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:99.775,133.579) {6};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:99.775,49.233) {7};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:93.715,90.369) {8};
\legend{}
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/subarray_14/angle_spectrum_subarray_14/angle_spectrum_subarray_14.tex <==
%!TEX root = ../../../../../../../../2023_EUCNC.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\definecolor{mycolor1}{rgb}{0.00000,1.00000,1.00000}%
\definecolor{mycolor2}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.852\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-30,
point meta max=0,
axis on top,
x dir=reverse,
xmin=-1.01123595505618,
xmax=181.011235955056,
xtick={  0,  45,  90, 135, 180},
%xlabel style={font=\color{white!15!black}},
xlabel={az. in deg},
y dir=reverse,
ymin=-1.52542372881356,
ymax=181.525423728814,
ytick={  0,  45,  90, 135, 180},
%ylabel style={font=\color{white!15!black}},
ylabel={el. in deg},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(1,1,1); rgb(255pt)=(0,0,0)},
%colorbar horizontal,
%colorbar style={at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=1.5mm,width=0.6\figurewidth,xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xlabel={ang.-spect. in dB},xtick distance={10}},
colorbar,
colorbar style={at={(1.02,0)},xticklabel pos=right,anchor=south west,major tick length=1mm,width=1.5mm,height=\figureheight, ylabel={ang.-spect. in dB}, yticklabel style={rotate=0,font=\footnotesize,xshift=-0.5mm}, ylabel style={yshift=2mm}, ytick distance={10}},
ylabel style={yshift=-2mm},
xlabel style={yshift=1.5mm},
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={angle spectrum}}
]
\addplot [forget plot] graphics [xmin=-1.01123595505618, xmax=181.011235955056, ymin=-1.52542372881356, ymax=181.525423728814] {\datapath/angle_spectrum_subarray_14-1.png};

\node[above, align=left, font={\scriptsize\color{red}}]%
at (axis cs:99.775,90.968) {1};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:28.093,90.613) {2};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:64.019,90.305) {3};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:161.288,90.2) {4};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:155.514,90.293) {5};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:99.775,133.579) {6};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:99.775,49.233) {7};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:93.715,90.369) {8};


\addplot[only marks, mark=+, mark options={}, mark size=1.5811pt, draw=red] table[]{\datapath/angle_spectrum_subarray_14-3.tsv};
\addlegendentry{data3}

\addplot[scatter, only marks, mark=o, color=mycolor2, mark options={}, scatter/use mapped color=mycolor2, visualization depends on={\thisrow{size} \as \perpointmarksize}, scatter/@pre marker code/.append style={/tikz/mark size=1.25*\perpointmarksize}] table[]{\datapath/angle_spectrum_subarray_14-2.tsv};
\addlegendentry{data2}

\addplot[scatter, only marks, mark=o, color=mycolor1, mark options={}, scatter/use mapped color=mycolor1, visualization depends on={\thisrow{size} \as \perpointmarksize}, scatter/@pre marker code/.append style={/tikz/mark size=1.25*\perpointmarksize}] table[]{\datapath/angle_spectrum_subarray_14-1.tsv};
\addlegendentry{data1}



\legend{}
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/subarray_14/signal_residual_subarray_14/signal_residual_subarray_14.tex <==
%!TEX root = ../../../../../../../../2023_EUCNC.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\definecolor{mycolor1}{rgb}{0.00000,1.00000,1.00000}%
\definecolor{mycolor2}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.852\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=21,%30,
%xlabel style={font=\color{white!15!black}},
xlabel={delay in m},
ymin=-15,%-20,
ymax=40,
%ylabel style={font=\color{white!15!black}},
ylabel={signal in dB},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1
ylabel style={yshift=-2mm},
xlabel style={yshift=1.5mm},
]
\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-1.tsv};
\addlegendentry{data1}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-2.tsv};
\addlegendentry{data2}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-3.tsv};
\addlegendentry{data3}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-4.tsv};
\addlegendentry{data4}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-5.tsv};
\addlegendentry{data5}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-6.tsv};
\addlegendentry{data6}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-7.tsv};
\addlegendentry{data7}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-8.tsv};
\addlegendentry{data8}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-9.tsv};
\addlegendentry{data9}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-10.tsv};
\addlegendentry{data10}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-11.tsv};
\addlegendentry{data11}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-12.tsv};
\addlegendentry{data12}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-13.tsv};
\addlegendentry{data13}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-14.tsv};
\addlegendentry{data14}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-15.tsv};
\addlegendentry{data15}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_14-16.tsv};
\addlegendentry{data16}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-17.tsv};
\addlegendentry{data17}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-18.tsv};
\addlegendentry{data18}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-19.tsv};
\addlegendentry{data19}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-20.tsv};
\addlegendentry{data20}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-21.tsv};
\addlegendentry{data21}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-22.tsv};
\addlegendentry{data22}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-23.tsv};
\addlegendentry{data23}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-24.tsv};
\addlegendentry{data24}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-25.tsv};
\addlegendentry{data25}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-26.tsv};
\addlegendentry{data26}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-27.tsv};
\addlegendentry{data27}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-28.tsv};
\addlegendentry{data28}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-29.tsv};
\addlegendentry{data29}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-30.tsv};
\addlegendentry{data30}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-31.tsv};
\addlegendentry{data31}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_14-32.tsv};
\addlegendentry{data32}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-33.tsv};
\addlegendentry{data33}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-34.tsv};
\addlegendentry{data34}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-35.tsv};
\addlegendentry{data35}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-36.tsv};
\addlegendentry{data36}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-37.tsv};
\addlegendentry{data37}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-38.tsv};
\addlegendentry{data38}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-39.tsv};
\addlegendentry{data39}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-40.tsv};
\addlegendentry{data40}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-41.tsv};
\addlegendentry{data41}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-42.tsv};
\addlegendentry{data42}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-43.tsv};
\addlegendentry{data43}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-44.tsv};
\addlegendentry{data44}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-45.tsv};
\addlegendentry{data45}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-46.tsv};
\addlegendentry{data46}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-47.tsv};
\addlegendentry{data47}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_14-48.tsv};
\addlegendentry{data48}

\addplot [color=red, dashed]
  table[]{\datapath/signal_residual_subarray_14-49.tsv};
\addlegendentry{data49}

\addplot [color=red, dashed]
  table[]{\datapath/signal_residual_subarray_14-50.tsv};
\addlegendentry{data50}

\addplot [color=red, dashed, forget plot]
  table[]{\datapath/signal_residual_subarray_14-51.tsv};
\addplot [color=red, dashed, forget plot]
  table[]{\datapath/signal_residual_subarray_14-52.tsv};
\addplot [color=red, dashed, forget plot]
  table[]{\datapath/signal_residual_subarray_14-53.tsv};
\addplot [color=red, dashed, forget plot]
  table[]{\datapath/signal_residual_subarray_14-54.tsv};
\addplot [color=red, dashed, forget plot]
  table[]{\datapath/signal_residual_subarray_14-55.tsv};
\addplot [color=red, dashed, forget plot]
  table[]{\datapath/signal_residual_subarray_14-56.tsv};
\addplot [color=red, line width=1.0pt, forget plot]
  table[]{\datapath/signal_residual_subarray_14-57.tsv};
\addplot [color=mycolor1, draw=none, mark=*, mark options={solid, fill=mycolor1, mycolor1}, forget plot]
  table[]{\datapath/signal_residual_subarray_14-58.tsv};
\addplot [color=mycolor2, draw=none, mark=*, mark options={solid, fill=mycolor2, mycolor2}, forget plot]
  table[]{\datapath/signal_residual_subarray_14-59.tsv};
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle,inner sep=0pt]%\node[right, align=left]
at (axis cs:3.308,29) {1};
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle,inner sep=0pt]%\node[right, align=left]
at (axis cs:5.221,28) {2};
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle,inner sep=0pt]%\node[right, align=left]
at (axis cs:10.514,27) {3};
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle,inner sep=0pt]%\node[right, align=left]
at (axis cs:15.981,26) {4};
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle,inner sep=0pt]%\node[right, align=left]
at (axis cs:10.924,25) {5};
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle,inner sep=0pt]%\node[right, align=left]
at (axis cs:4.566,24) {6};
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle,inner sep=0pt]%\node[right, align=left]
at (axis cs:4.368,23) {7};
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle,inner sep=0pt]%\node[right, align=left]
at (axis cs:8.668,22) {8};
\legend{}
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/subarray_500/angle_spectrum_residual_subarray_500/angle_spectrum_residual_subarray_500.tex <==
%!TEX root = ../../../../../../../../main_d12.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.852\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-30,
point meta max=0,
axis on top,
x dir=reverse,
xmin=-1.01123595505618,
xmax=181.011235955056,
xtick={  0,  45,  90, 135, 180},
%xlabel style={font=\color{white!15!black}},
xlabel={az. in deg},
y dir=reverse,
ymin=-1.52542372881356,
ymax=181.525423728814,
ytick={  0,  45,  90, 135, 180},
%ylabel style={font=\color{white!15!black}},
ylabel={el. in deg},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(1,1,1); rgb(255pt)=(0,0,0)},
colorbar horizontal,
colorbar style={at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=1.5mm,width=0.6\figurewidth,xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xlabel={ang.-spect. in dB},xtick distance={10}},
%colorbar,
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={res. angle spectrum}}
]
\addplot [forget plot] graphics [xmin=-1.01123595505618, xmax=181.011235955056, ymin=-1.52542372881356, ymax=181.525423728814] {\datapath/angle_spectrum_residual_subarray_500-1.png};
\addplot[only marks, mark=+, mark options={}, mark size=1.5811pt, draw=red] table[]{\datapath/angle_spectrum_residual_subarray_500-1.tsv};
\addlegendentry{data1}

\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:61.532,90.863) {1};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:19.52,90.435) {2};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:53.729,90.273) {3};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:158.183,90.232) {4};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:149.256,90.361) {5};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:61.532,130.326) {6};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:61.532,52.436) {7};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:78.45,90.363) {8};
\legend{}
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/subarray_500/angle_spectrum_subarray_500/angle_spectrum_subarray_500.tex <==
%!TEX root = ../../../../../../../../main_d12.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\definecolor{mycolor1}{rgb}{0.00000,1.00000,1.00000}%
\definecolor{mycolor2}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.852\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-30,
point meta max=0,
axis on top,
x dir=reverse,
xmin=-1.01123595505618,
xmax=181.011235955056,
xtick={  0,  45,  90, 135, 180},
%xlabel style={font=\color{white!15!black}},
xlabel={az. in deg},
y dir=reverse,
ymin=-1.52542372881356,
ymax=181.525423728814,
ytick={  0,  45,  90, 135, 180},
%ylabel style={font=\color{white!15!black}},
ylabel={el. in deg},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(1,1,1); rgb(255pt)=(0,0,0)},
colorbar horizontal,
colorbar style={at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=1.5mm,width=0.6\figurewidth,xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xlabel={ang.-spect. in dB},xtick distance={10}},
%colorbar,
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={angle spectrum}}
]
\addplot [forget plot] graphics [xmin=-1.01123595505618, xmax=181.011235955056, ymin=-1.52542372881356, ymax=181.525423728814] {\datapath/angle_spectrum_subarray_500-1.png};


\addplot[only marks, mark=+, mark options={}, mark size=1.5811pt, draw=red] table[]{\datapath/angle_spectrum_subarray_500-3.tsv};
\addlegendentry{data3}

\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:61.532,90.863) {1};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:19.52,90.435) {2};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:53.729,90.273) {3};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:158.183,90.232) {4};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:149.256,90.361) {5};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:61.532,130.326) {6};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:61.532,52.436) {7};
\node[above, align=left, font={\scriptsize\color{red}}]%\node[right, align=left, font=\color{red}]
at (axis cs:78.45,90.363) {8};


\addplot[scatter, only marks, mark=o, color=mycolor2, mark options={}, scatter/use mapped color=mycolor2, visualization depends on={\thisrow{size} \as \perpointmarksize}, scatter/@pre marker code/.append style={/tikz/mark size=1.25*\perpointmarksize}] table[]{\datapath/angle_spectrum_subarray_500-2.tsv};
\addlegendentry{data2}

\addplot[scatter, only marks, mark=o, color=mycolor1, mark options={}, scatter/use mapped color=mycolor1, visualization depends on={\thisrow{size} \as \perpointmarksize}, scatter/@pre marker code/.append style={/tikz/mark size=1.25*\perpointmarksize}] table[]{\datapath/angle_spectrum_subarray_500-1.tsv};
\addlegendentry{data1}


\legend{}
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/subarray_500/signal_residual_subarray_500/signal_residual_subarray_500.tex <==
%!TEX root = ../../../../../../../../main_d12.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\definecolor{mycolor1}{rgb}{0.00000,1.00000,1.00000}%
\definecolor{mycolor2}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.852\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=21,%30,
%xlabel style={font=\color{white!15!black}},
xlabel={delay in m},
ymin=-10,%-20,
ymax=40,
%ylabel style={font=\color{white!15!black}},
ylabel={signal in dB},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1
]
\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-1.tsv};
\addlegendentry{data1}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-2.tsv};
\addlegendentry{data2}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-3.tsv};
\addlegendentry{data3}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-4.tsv};
\addlegendentry{data4}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-5.tsv};
\addlegendentry{data5}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-6.tsv};
\addlegendentry{data6}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-7.tsv};
\addlegendentry{data7}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-8.tsv};
\addlegendentry{data8}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-9.tsv};
\addlegendentry{data9}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-10.tsv};
\addlegendentry{data10}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-11.tsv};
\addlegendentry{data11}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-12.tsv};
\addlegendentry{data12}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-13.tsv};
\addlegendentry{data13}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-14.tsv};
\addlegendentry{data14}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-15.tsv};
\addlegendentry{data15}

\addplot [color=black]
  table[]{\datapath/signal_residual_subarray_500-16.tsv};
\addlegendentry{data16}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-17.tsv};
\addlegendentry{data17}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-18.tsv};
\addlegendentry{data18}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-19.tsv};
\addlegendentry{data19}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-20.tsv};
\addlegendentry{data20}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-21.tsv};
\addlegendentry{data21}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-22.tsv};
\addlegendentry{data22}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-23.tsv};
\addlegendentry{data23}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-24.tsv};
\addlegendentry{data24}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-25.tsv};
\addlegendentry{data25}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-26.tsv};
\addlegendentry{data26}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-27.tsv};
\addlegendentry{data27}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-28.tsv};
\addlegendentry{data28}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-29.tsv};
\addlegendentry{data29}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-30.tsv};
\addlegendentry{data30}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-31.tsv};
\addlegendentry{data31}

\addplot [color=green]
  table[]{\datapath/signal_residual_subarray_500-32.tsv};
\addlegendentry{data32}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-33.tsv};
\addlegendentry{data33}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-34.tsv};
\addlegendentry{data34}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-35.tsv};
\addlegendentry{data35}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-36.tsv};
\addlegendentry{data36}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-37.tsv};
\addlegendentry{data37}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-38.tsv};
\addlegendentry{data38}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-39.tsv};
\addlegendentry{data39}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-40.tsv};
\addlegendentry{data40}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-41.tsv};
\addlegendentry{data41}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-42.tsv};
\addlegendentry{data42}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-43.tsv};
\addlegendentry{data43}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-44.tsv};
\addlegendentry{data44}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-45.tsv};
\addlegendentry{data45}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-46.tsv};
\addlegendentry{data46}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-47.tsv};
\addlegendentry{data47}

\addplot [color=blue]
  table[]{\datapath/signal_residual_subarray_500-48.tsv};
\addlegendentry{data48}

\addplot [color=red, dashed]
  table[]{\datapath/signal_residual_subarray_500-49.tsv};
\addlegendentry{data49}

\addplot [color=red, dashed]
  table[]{\datapath/signal_residual_subarray_500-50.tsv};
\addlegendentry{data50}

\addplot [color=red, dashed, forget plot]
  table[]{\datapath/signal_residual_subarray_500-51.tsv};
\addplot [color=red, dashed, forget plot]
  table[]{\datapath/signal_residual_subarray_500-52.tsv};
\addplot [color=red, dashed, forget plot]
  table[]{\datapath/signal_residual_subarray_500-53.tsv};
\addplot [color=red, dashed, forget plot]
  table[]{\datapath/signal_residual_subarray_500-54.tsv};
\addplot [color=red, dashed, forget plot]
  table[]{\datapath/signal_residual_subarray_500-55.tsv};
\addplot [color=red, dashed, forget plot]
  table[]{\datapath/signal_residual_subarray_500-56.tsv};
\addplot [color=red, line width=1.0pt, forget plot]
  table[]{\datapath/signal_residual_subarray_500-57.tsv};
  
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle]%\node[right, align=left]
at (axis cs:3.709,29) {1};
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle]%\node[right, align=left]
at (axis cs:7.358,28) {2};
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle]%\node[right, align=left]
at (axis cs:11.723,27) {3};
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle]%\node[right, align=left]
at (axis cs:13.795,26) {4};
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle]%\node[right, align=left]
at (axis cs:8.857,25) {5};
\node[below, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle]%\node[right, align=left]
at (axis cs:4.864,24) {6};
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle]%\node[right, align=left]
at (axis cs:4.678,23) {7};
\node[above, align=left, font={\scriptsize\color{red}},draw=red,fill=white,circle]%\node[right, align=left]
at (axis cs:8.829,22) {8};
  
\addplot [color=mycolor1, draw=none, mark=*, mark options={solid, fill=mycolor1, mycolor1}, forget plot]
  table[]{\datapath/signal_residual_subarray_500-58.tsv};
\addplot [color=mycolor2, draw=none, mark=*, mark options={solid, fill=mycolor2, mycolor2}, forget plot]
  table[]{\datapath/signal_residual_subarray_500-59.tsv};

\legend{}
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA1_MPC_amplitude_PL-comp_img/VA1_MPC_amplitude_PL-comp_img.tex <==
%!TEX root = ../../../../../../../2023_EUCNC.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-49.4450205994778,
point meta max=-39.4450205994778,
axis on top,
xmin=0.5,
xmax=14.5,
%xlabel style={font=\color{white!15!black}},
xlabel={hor. idx.},
ymin=0.5,
ymax=9.5,
%ylabel style={font=\color{white!15!black}},
ylabel={vert. idx.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
major tick length=0.75mm,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
%colorbar horizontal,
%colorbar style={at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=1.5mm,width=0.5\figurewidth,xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xlabel=est. amp. in dB,xtick distance={4}}
%colorbar style={at={(1.02,1)},xticklabel pos=right,anchor=north west,major tick length=1mm,width=2mm,height=0.6\figureheight,yticklabel style={rotate=0,font=\footnotesize,xshift=0mm},ylabel=est. amp. in dB}
%colorbar,
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
colorbar,
colorbar style={at={(1.02,0)},xticklabel pos=right,anchor=south west,major tick length=1mm,width=1.5mm,height=\figureheight,yticklabel style={rotate=90,font=\footnotesize,xshift=0mm},ylabel=est. amp. in dB, ylabel style={yshift=2mm}, ytick distance={4}},
ylabel style={yshift=-1.5mm},
xlabel style={yshift=1.5mm},
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA1_MPC_amplitude_PL-comp_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA1_MPC_visibility_img/VA1_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=0.857\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=14.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=9.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA1_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA2_MPC_amplitude_PL-comp_img/VA2_MPC_amplitude_PL-comp_img.tex <==
%!TEX root = ../../../../../../../main_d12.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{every axis/.append style={
    label style={font=\footnotesize},
    legend style={font=\footnotesize},
    tick label style={font=\footnotesize},
    xticklabel={
      % test if the x value is below zero
      \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
      \else
      % if no, print as usual
      \pgfmathprintnumber{\tick}
      \fi
}}}

\begin{tikzpicture}

\begin{axis}[%
width=0.926\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-52.9214905977668,
point meta max=-42.9214905977668,
axis on top,
xmin=0.5,
xmax=14.5,
%xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=9.5,
%ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
colorbar horizontal,
colorbar style={at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=1.5mm,width=0.5\figurewidth,xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xlabel=est. amp. in dB,xtick distance={4}}
%colorbar style={at={(1.02,1)},xticklabel pos=right,anchor=north west,major tick length=1mm,width=2mm,height=0.6\figureheight,yticklabel style={rotate=0,font=\footnotesize,xshift=0mm},ylabel=est. amp. in dB}
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA2_MPC_amplitude_PL-comp_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA2_MPC_visibility_img/VA2_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=0.857\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=14.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=9.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA2_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA3_MPC_amplitude_PL-comp_img/VA3_MPC_amplitude_PL-comp_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=0.857\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-59.9022938992332,
point meta max=-49.9022938992332,
axis on top,
xmin=0.5,
xmax=14.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=9.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA3_MPC_amplitude_PL-comp_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA3_MPC_visibility_img/VA3_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=0.857\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=14.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=9.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA3_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA4_MPC_amplitude_PL-comp_img/VA4_MPC_amplitude_PL-comp_img.tex <==
%!TEX root = ../../../../../../../main_d12.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=0.926\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-58.5491094521124,
point meta max=-48.5491094521124,
axis on top,
xmin=0.5,
xmax=14.5,
%xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=9.5,
%ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
 unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
colorbar horizontal,
colorbar style={at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=1.5mm,width=0.5\figurewidth,xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xlabel=est. amp. in dB,xtick distance={4}}
%colorbar,
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA4_MPC_amplitude_PL-comp_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA4_MPC_visibility_img/VA4_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=0.857\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=14.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=9.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA4_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA5_MPC_amplitude_PL-comp_img/VA5_MPC_amplitude_PL-comp_img.tex <==
%!TEX root = ../../../../../../../2023_EUCNC.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
    % if yes, calculate the absolute value
    \pgfmathparse{abs(\tick)}%
    % and print first a minus sign in a zero-width box, followed by the absolute value
    \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
    \else
    % if no, print as usual
    \pgfmathprintnumber{\tick}
    \fi
}}}

\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-64.1870341009192,
point meta max=-54.1870341009192,
axis on top,
xmin=0.5,
xmax=14.5,
%xlabel style={font=\color{white!15!black}},
xlabel={hor. idx.},
ymin=0.5,
ymax=9.5,
%ylabel style={font=\color{white!15!black}},
ylabel={vert. idx.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
major tick length=0.75mm,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
 unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
%colorbar horizontal,
%colorbar style={at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=1.5mm,width=0.5\figurewidth,xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xlabel=est. amp. in dB,xtick distance={4}}
%colorbar style={at={(1.02,1)},xticklabel pos=right,anchor=north west,major tick length=1mm,width=2mm,height=0.6\figureheight,yticklabel style={rotate=0,font=\footnotesize,xshift=0mm},ylabel=est. amp. in dB}
%colorbar style={at={(1.02,1)},xticklabel pos=right,anchor=north west,major tick length=1mm,width=2mm,height=0.6\figureheight,yticklabel style={rotate=0,font=\footnotesize,xshift=0mm},ylabel=est. amp. in dB}
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
colorbar,
colorbar style={at={(1.02,0)},xticklabel pos=right,anchor=south west,major tick length=1mm,width=1.5mm,height=\figureheight,yticklabel style={rotate=90,font=\footnotesize,xshift=0mm},ylabel=est. amp. in dB, ylabel style={yshift=2mm}, ytick distance={4}},
ylabel style={yshift=-1.5mm},
xlabel style={yshift=1.5mm},
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA5_MPC_amplitude_PL-comp_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA5_MPC_visibility_img/VA5_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=0.857\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=14.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=9.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA5_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA6_MPC_amplitude_PL-comp_img/VA6_MPC_amplitude_PL-comp_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=0.857\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-63.5294915059862,
point meta max=-53.5294915059862,
axis on top,
xmin=0.5,
xmax=14.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=9.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA6_MPC_amplitude_PL-comp_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA6_MPC_visibility_img/VA6_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=0.857\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=14.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=9.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA6_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA7_MPC_amplitude_PL-comp_img/VA7_MPC_amplitude_PL-comp_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=0.857\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-70.7204760131126,
point meta max=-60.7204760131126,
axis on top,
xmin=0.5,
xmax=14.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=9.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA7_MPC_amplitude_PL-comp_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA7_MPC_visibility_img/VA7_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=0.857\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=14.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=9.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA7_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA8_MPC_amplitude_PL-comp_img/VA8_MPC_amplitude_PL-comp_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=0.857\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-50.4733273576864,
point meta max=-40.4733273576864,
axis on top,
xmin=0.5,
xmax=14.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=9.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA8_MPC_amplitude_PL-comp_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny8_Nz8/portal2_pos1/VA8_MPC_visibility_img/VA8_MPC_visibility_img.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=0.857\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=14.5,
xlabel style={font=\color{white!15!black}},
xlabel={subarray index hor.},
ymin=0.5,
ymax=9.5,
ylabel style={font=\color{white!15!black}},
ylabel={subarray index vert.},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
% unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar,
colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=14.5, ymin=0.5, ymax=9.5] {\datapath/VA8_MPC_visibility_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-11_VNA_corridor/portal2_pos1/VA1_MPC_amplitude_PL-comp_img/VA1_MPC_amplitude_PL-comp_img.tex <==
%!TEX root = ../../../../../../2023_EUCNC.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-43.4864488639062,
point meta max=-33.4864488639062,
axis on top,
xmin=0.5,
xmax=22.5,
%xlabel style={font=\color{white!15!black}},
xlabel={hor. idx},%{subarray index hor.},
ymin=0.5,
ymax=8.5,
%ylabel style={font=\color{white!15!black}},
ylabel={vert. idx},%{subarray index vert.},
axis background/.style={fill=white},
%title style={font=\bfseries},
%title={segments:},
xmajorgrids,
ymajorgrids,
major tick length=0.75mm,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
%colorbar horizontal,
%colorbar style={at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=1.5mm,width=0.5\figurewidth,xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xlabel=est. amp. in dB,xtick distance={4}}
colorbar,
colorbar style={at={(1.02,0)},xticklabel pos=right,anchor=south west,major tick length=1mm,width=1.5mm,yticklabel style={rotate=90,font=\footnotesize,xshift=0mm},ylabel=est. amp. in dB, ylabel style={yshift=2mm}, ytick distance={4}},
ylabel style={yshift=-1.5mm},
xlabel style={yshift=1.5mm},
%colorbar,
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=22.5, ymin=0.5, ymax=8.5] {\datapath/VA1_MPC_amplitude_PL-comp_img-1.png};

\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-11_VNA_corridor/portal2_pos1/VA1_directpath_path__model_vis_img/VA1_directpath_path__model_vis_img.tex <==
%!TEX root = ../../../../../../2023_EUCNC.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=22.5,
%xlabel style={font=\color{white!15!black}},
xlabel={hor. idx},%{subarray index hor.},
ymin=0.5,
ymax=8.5,
%ylabel style={font=\color{white!15!black}},
ylabel={vert. idx},%{subarray index vert.},
axis background/.style={fill=white},
%title style={font=\bfseries},
%title={},
xmajorgrids,
ymajorgrids,
major tick length=0.75mm,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar sampled,
colorbar style={samples=3,at={(1.02,0)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=6mm,width=1.5mm,ytick={0.25,0.75},yticklabels={invis.,vis.},xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xtick distance={1}},%,point meta min=0,point meta max=1}
%colorbar style={samples=3,at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=6mm,width=1.5mm,ytick={0.25,0.75},yticklabels={not visible,visible},xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xtick distance={1}},%,point meta min=0,point meta max=1}
ylabel style={yshift=-1.5mm},
xlabel style={yshift=1.5mm},
%colorbar,
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={geom. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=22.5, ymin=0.5, ymax=8.5] {\datapath/VA1_directpath_path__model_vis_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-11_VNA_corridor/portal2_pos1/VA4_MPC_amplitude_PL-comp_img/VA4_MPC_amplitude_PL-comp_img.tex <==
%!TEX root = ../../../../../../2023_EUCNC.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-43.8357648364306,
point meta max=-33.8357648364306,
axis on top,
xmin=0.5,
xmax=22.5,
%xlabel style={font=\color{white!15!black}},
xlabel={hor. idx.},%{subarray index hor.},
ymin=0.5,
ymax=8.5,
%ylabel style={font=\color{white!15!black}},
ylabel={ver. idx.},%{subarray index vert.},
axis background/.style={fill=white},
%title style={font=\bfseries},
%title={segments:  92},
xmajorgrids,
ymajorgrids,
major tick length=0.75mm,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
%colorbar,
%colorbar horizontal,
%colorbar style={at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=1.5mm,width=0.5\figurewidth,xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xlabel=est. amp. in dB,xtick distance={4}}
colorbar,
colorbar style={at={(1.02,0)},xticklabel pos=right,anchor=south west,major tick length=1mm,width=1.5mm,yticklabel style={rotate=90,font=\footnotesize,xshift=0mm},ylabel=est. amp. in dB, ylabel style={yshift=2mm}, ytick distance={4}},
ylabel style={yshift=-1.5mm},
xlabel style={yshift=1.5mm},
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=22.5, ymin=0.5, ymax=8.5] {\datapath/VA4_MPC_amplitude_PL-comp_img-1.png};

\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-11_VNA_corridor/portal2_pos1/VA4_wallsouth_path_92_model_vis_img/VA4_wallsouth_path_92_model_vis_img.tex <==
%!TEX root = ../../../../../../main_d12.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=0.606\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=0,
point meta max=1,
axis on top,
xmin=0.5,
xmax=22.5,
%xlabel style={font=\color{white!15!black}},
xlabel={hor. idx.},%{subarray index hor.},
ymin=0.5,
ymax=8.5,
%ylabel style={font=\color{white!15!black}},
ylabel={vert. idx.},%{subarray index vert.},
axis background/.style={fill=white},
%title style={font=\bfseries},
%title={92},
xmajorgrids,
ymajorgrids,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.2422,0.1504,0.6603)},
colorbar sampled,
colorbar style={samples=3,at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=6mm,width=1.5mm,ytick={0.25,0.75},yticklabels={not visible,visible},xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xtick distance={1}},%,point meta min=0,point meta max=1}
%colorbar,
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={geom. vis.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=22.5, ymin=0.5, ymax=8.5] {\datapath/VA4_wallsouth_path_92_model_vis_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/results/sbl/2022-11_VNA_corridor/portal2_pos1/VA5_MPC_amplitude_PL-comp_img/VA5_MPC_amplitude_PL-comp_img.tex <==
%!TEX root = ../../../../../../2023_EUCNC.tex

% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
 
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\footnotesize},
  tick label style={font=\footnotesize},
  xticklabel={
    % test if the x value is below zero
    \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
     % if no, print as usual
      \pgfmathprintnumber{\tick}
   \fi
}}}
 
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
point meta min=-50.0914661006571,
point meta max=-40.0914661006571,
axis on top,
xmin=0.5,
xmax=22.5,
%xlabel style={font=\color{white!15!black}},
xlabel={hor. idx.},%{subarray index hor.},
ymin=0.5,
ymax=8.5,
%ylabel style={font=\color{white!15!black}},
ylabel={vert. idx.},%{subarray index vert.},
axis background/.style={fill=white},
%title style={font=\bfseries},
%title={segments:  93},
xmajorgrids,
ymajorgrids,
major tick length=0.75mm,
grid style=dotted,
legend style={legend cell align=left, align=left, draw=white!15!black},
%extraAxisOptions,
 unit vector ratio=1 1 1,
colormap={mymap}{[1pt] rgb(0pt)=(0.9769,0.9839,0.0805); rgb(1pt)=(0.960065,0.919778,0.138513); rgb(2pt)=(0.972487,0.851822,0.170039); rgb(3pt)=(0.99583,0.784087,0.206396); rgb(4pt)=(0.974183,0.729983,0.240235); rgb(5pt)=(0.876009,0.73807,0.163478); rgb(6pt)=(0.752635,0.764204,0.175091); rgb(7pt)=(0.607761,0.788896,0.26853); rgb(8pt)=(0.450713,0.802217,0.387143); rgb(9pt)=(0.307896,0.798696,0.505248); rgb(10pt)=(0.206843,0.781061,0.60543); rgb(11pt)=(0.135809,0.757291,0.6878); rgb(12pt)=(0.0091913,0.732587,0.762583); rgb(13pt)=(0.054713,0.700157,0.83063); rgb(14pt)=(0.115917,0.657465,0.881052); rgb(15pt)=(0.146526,0.6075,0.909004); rgb(16pt)=(0.175852,0.553443,0.948983); rgb(17pt)=(0.188526,0.494822,0.9855); rgb(18pt)=(0.249787,0.428622,0.997791); rgb(19pt)=(0.276183,0.365713,0.9825); rgb(20pt)=(0.2814,0.305435,0.945196); rgb(21pt)=(0.276739,0.244439,0.885183); rgb(22pt)=(0.262948,0.193548,0.783748); rgb(23pt)=(0.2422,0.1504,0.6603)},
%colorbar horizontal,
%colorbar style={at={(0,1.05)},xticklabel pos=right,anchor=south west,major tick length=1mm,height=1.5mm,width=0.5\figurewidth,xticklabel style={rotate=0,font=\footnotesize,xshift=0mm},xlabel=est. amp. in dB,xtick distance={4}}
colorbar,
colorbar style={at={(1.02,0)},xticklabel pos=right,anchor=south west,major tick length=1mm,width=1.5mm,yticklabel style={rotate=90,font=\footnotesize,xshift=0mm},ylabel=est. amp. in dB, ylabel style={yshift=2mm}, ytick distance={4}},
ylabel style={yshift=-1.5mm},
xlabel style={yshift=1.5mm},
%colorbar style={ylabel style={font=\color{white!15!black}}, ylabel={est. amp.}}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=22.5, ymin=0.5, ymax=8.5] {\datapath/VA5_MPC_amplitude_PL-comp_img-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/sbl_figure.tex <==
\begin{figure*}[t!]
  % \flushright%
  \centering
  \subfloat[angle-spectrum]{%\hspace{-5mm}
    \setlength{\figurewidth}{0.2\textwidth}
    \setlength{\figureheight}{0.12\textwidth}
    \def\datapath{./figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/subarray_14/angle_spectrum_subarray_14}
    \input{\datapath/angle_spectrum_subarray_14.tex}
    \label{fig:meas:tug:static:medium:pos1:4x4:sb14:angle}
  }%\hspace{1mm}
  \subfloat[residual angle-spectrum]{%\hspace{-5mm}
    \setlength{\figurewidth}{0.2\textwidth}
    \setlength{\figureheight}{0.12\textwidth}
    \def\datapath{./figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/subarray_14/angle_spectrum_residual_subarray_14}
    \input{\datapath/angle_spectrum_residual_subarray_14.tex}
    \label{fig:meas:tug:static:medium:pos1:4x4:sb14:residual_angle}
  }%\hspace{1mm}
  \subfloat[time-domain signals]{%\hspace{-5mm}
    \setlength{\figurewidth}{0.2\textwidth}
    \setlength{\figureheight}{0.12\textwidth}
    \def\datapath{./figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/subarray_14/signal_residual_subarray_14}
    \input{\datapath/signal_residual_subarray_14.tex}
    \label{fig:meas:tug:static:medium:pos1:4x4:sb14:signal}
  }
  
%  \subfloat[angle-spectrum for M1 and subarray 500 of dim. $4\times 4$]{%\hspace{-5mm}
%    \setlength{\figurewidth}{0.255\textwidth}
%    \setlength{\figureheight}{0.2\textwidth}
%    \def\datapath{./figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/subarray_500/angle_spectrum_subarray_500}
%    \input{\datapath/angle_spectrum_subarray_500.tex}
%    \label{fig:meas:tug:static:medium:pos1:4x4:sb500:angle}
%  }\hspace{1mm}
%  \subfloat[residual angle-spectrum for M1 and subarray 500 of dim. $4\times 4$]{%\hspace{-5mm}
%    \setlength{\figurewidth}{0.255\textwidth}
%    \setlength{\figureheight}{0.2\textwidth}
%    \def\datapath{./figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/subarray_500/angle_spectrum_residual_subarray_500}
%    \input{\datapath/angle_spectrum_residual_subarray_500.tex}
%    \label{fig:meas:tug:static:medium:pos1:4x4:sb500:residual_angle}
%  }\hspace{1mm}
%  \subfloat[time-domain signals for M1 and subarray 500 of dim. $4\times 4$]{%\hspace{-5mm}
%    \setlength{\figurewidth}{0.255\textwidth}
%    \setlength{\figureheight}{0.2\textwidth}
%    \def\datapath{./figures/results/sbl/2022-08_VNA_full_array/array-Nx1_Ny112_Nz75_signal-bw500MHz_fc6950MHz_subarray_sbl-Nx1_Ny4_Nz4/portal2_pos1/subarray_500/signal_residual_subarray_500}
%    \input{\datapath/signal_residual_subarray_500.tex}
%    \label{fig:meas:tug:static:medium:pos1:4x4:sb500:signal}
%  }
  
  \caption{\Gls{sbl} performance showing estimated components over the angle-spectrum, residual angle-spectrum and residual time-domain signals. Results are shown for $4\times 4$ subarrays with $500~\mathrm{MHz}$ bandwidth. \com{tw: not needed}}\label{fig:meas:sbl}
\end{figure*}


==> figures/system_setup_v1.tex <==
%!TEX root= ../2023_EUCNC.tex

% [B] changes: 		"3.0"		--> "1.5"
% [B] changes: 		"2.0"		--> "1.0"
% [B] changes: 		") {"		--> ") {\footnotesize "
% [B] changes:		"\addplot3 [color=mycolor2, line width=1.0pt]"
%				--> "\addplot3 [color=mycolor2, line width=1.0pt, rounded corners=0.1pt, line cap=round]"
% [B] changes:		"\addplot3 [color=mycolor1, line width=\lwA]"
% 				--> "\addplot3 [color=mycolor1, line width=\lwA, rounded corners=0.1pt, line cap=round]"

\pgfplotsset{every axis/.append style={
    label style={font=\footnotesize},
    legend style={font=\footnotesize},
    tick label style={font=\footnotesize},
    xticklabel={
      % test if the x value is below zero
      \ifdim \tick pt < 0pt
      % if yes, calculate the absolute value
      \pgfmathparse{abs(\tick)}%
      % and print first a minus sign in a zero-width box, followed by the absolute value
      \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
      \else
      % if no, print as usual
      \pgfmathprintnumber{\tick}
      \fi
}}}


\definecolor{mycolor1}{rgb}{0.5,0.5,0.5}%{0.52157,0.21961,0.35294}%
\definecolor{mycolor2}{rgb}{0.4,0.4,1}%
\definecolor{mycolor2text}{rgb}{0.1,0.1,1}%
\definecolor{mycolor3}{rgb}{1.00000,0.00000,1.00000}%
\definecolor{mycolor4}{rgb}{0.36471,0.42745,0.26667}%		
%
\def\lwA{0.5pt}
\def\lwB{0.75pt}
\def\wallopac{0.3}
\def\annopac{1}
\def\vaannopac{0.5}
\def\textangle{0}

\tikzset{
coordinatesystem/.pic={
  \draw[red]   (0,0,0) -- (0,0,1);
  \draw[green] (0,0,0) -- (0,1,0);
  \draw[blue]  (0,0,0) -- (1,0,0);
}
}


\begin{tikzpicture}

\begin{axis}[%
width=0.95\figurewidth,
height=0.9\figureheight,
at={(0\figurewidth,0\figureheight)},
%scale only axis,
clip mode=individual,
plot box ratio=1 1 0.9,%1.875 2.625 1,
xmin=3,
xmax=12.3,
xtick distance={3},				% [B]
ytick distance={3},				% [B]
ztick distance={1},				% [B]
%xlabel style={font=\color{white!15!black}},
xlabel={$x$ in m},
ymin=0,
ymax=9,
%ylabel style={font=\color{white!15!black}},
ylabel={$y$ in m},
zmin=0,
zmax=3,
%zlabel style={font=\color{white!15!black}},
zlabel={$z$ in m},
view={-130}{50},
%view={55}{50},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
zmajorgrids,
grid style=dotted,
major tick length=0.75mm,
ylabel style={yshift=5mm},
xlabel style={yshift=5mm},
%unit direction vector=1 1 1,
legend style={at={(0,0.8)},anchor=south,legend cell align=left, align=left, draw=none,fill=none},
]



\addlegendimage{->,black,solid,mark=o,mark options={mark size=1.5pt,color=black}}
\addlegendentry{visible path}

\addlegendimage{->,red!50!white,dashed,mark=x,mark options={mark size=2.125pt,color=red!50!white,solid}}
\addlegendentry{invisible path}



%VA front wall
\addplot3[area legend,densely dashed,draw=mycolor2, fill=mycolor2, fill opacity=0.1, forget plot]
table[row sep=crcr] {%
  x	y	z\\
  9.8	0	1.7\\
  9.8	0	1.7\\
  9.8	0	0.3\\
  12.2	0	0.3\\
  12.2	0	0.3\\
  12.2	0	1.7\\
  9.8	0	1.7\\
}--cycle;

\addplot3 [color=red,densely dashed, line width=1.0pt, line cap=round]
table[row sep=crcr] {%
  11	0	1\\
  10	0	1\\
};
%\node[right, align=left, font={\tiny\color{black!20!red}}] at (axis cs:10,0,1) {$x$};
\addplot3 [color=green,densely dashed, line width=1.0pt, line cap=round]
table[row sep=crcr] {%
  11	0	1\\
  11	1	1\\
};
%\node[left, align=left, font={\tiny\color{black!20!green}}] at (axis cs:11,1,1) {$y$};
\addplot3 [color=blue,densely dashed, line width=1.0pt, line cap=round]
table[row sep=crcr] {%
  11	0	1\\
  11	0	2\\
};
% \node[above, align=left, font={\tiny\color{black!20!blue}}] at (axis cs:11,0,2) {$z$};


\addplot3 [densely dotted,color=mycolor2, line width=\lwA, line cap=round]
table[row sep=crcr] {%
  9.8	0	0.3\\
  9.8	0	0\\
};
\addplot3 [densely dotted,color=mycolor2, line width=\lwA, line cap=round]
table[row sep=crcr] {%
  12.2	0	0.3\\
  12.2	0	0\\
};

%%left wall
%\addplot3[area legend, line width=\lwA, draw=mycolor1, fill=mycolor1, fill opacity=0.2, forget plot]%, rounded corners=0.1pt, line cap=round]
%table[row sep=crcr] {%
%x	y	z\\
%3	0	0\\
%3	9	0\\
%3	9	3\\
%3	0	3\\
%3	0	0\\
%}--cycle;



%right wall / reflection wall
\addplot3[area legend, line width=\lwA, draw=mycolor1, fill=mycolor1, fill opacity=\wallopac, forget plot]%, rounded corners=0.1pt, line cap=round]
table[row sep=crcr] {%
x	y	z\\
8	0	0\\
8	4.25	0\\
8	4.25	3\\
8	0	3\\
8	0	0\\
}--cycle;



%array wall
\addplot3[area legend, line width=\lwA, draw=mycolor1, fill=mycolor1, fill opacity=\wallopac, forget plot]%, rounded corners=0.1pt, line cap=round]
table[row sep=crcr] {%
x	y	z\\
3	0	0\\
8	0	0\\
8	0	3\\
3	0	3\\
3	0	0\\
}--cycle;

 

%back wall
%\addplot3[area legend, line width=\lwA, draw=mycolor1, fill=mycolor1, fill opacity=0.2, forget plot]%, rounded corners=0.1pt, line cap=round]
%table[row sep=crcr] {%
%x	y	z\\
%3	9	0\\
%8	9	0\\
%8	9	3\\
%3	9	3\\
%3	9	0\\
%}--cycle;

 
 
%floor
\addplot3[area legend, line width=\lwA, draw=mycolor1, fill=mycolor1, fill opacity=\wallopac, forget plot]%, rounded corners=0.1pt, line cap=round]
table[row sep=crcr] {%
x	y	z\\
3	0	0\\
3	9	0\\
8	9	0\\
8	0	0\\
3	0	0\\
}--cycle;


%segment highlight 
\addplot3[solid, area legend, line width=\lwB, draw=green!60!black, forget plot]%, rounded corners=0.1pt, line cap=round]
table[row sep=crcr] {%
  x	y	z\\
  8	0	0\\
  8	4.25	0\\
  8	4.25	3\\
  8	0	3\\
  8	0	0\\
}--cycle;
\node[green!60!black,font=\tiny,anchor=north,yshift=-0.75mm,rotate=\textangle] at (axis cs:8,2,0) {$k$th segment};



%physical anchor
\addplot3[area legend, solid, line width=0.7pt, draw=mycolor2, fill=mycolor2, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
  x	y	z\\
  3.8	0	1.7\\
  3.8	0	1.7\\
  3.8	0	0.3\\
  6.2	0	0.3\\
  6.2	0	0.3\\
  6.2	0	1.7\\
  3.8	0	1.7\\
}--cycle;

\addplot3 [color=red, line width=1.0pt, line cap=round] table[row sep=crcr] {%
5	0	1\\
6	0	1\\
};

%\node[right, align=left, font={\scriptsize\color{black!20!red}}] at (axis cs:6,0,1) {x};
\addplot3 [color=green, line width=1.0pt, line cap=round]
 table[row sep=crcr] {%
5	0	1\\
5	1	1\\
};
% \node[right, align=left, font={\scriptsize\color{black!20!green}}] at (axis cs:5,1,1) {y};
\addplot3 [color=blue, line width=1.0pt, line cap=round]
 table[row sep=crcr] {%
5	0	1\\
5	0	2\\
};
% \node[right, align=left, font={\scriptsize\color{black!20!blue}}] at (axis cs:5,0,2) {z};


\addplot3 [densely dotted,color=mycolor2, line width=\lwA, line cap=round]
table[row sep=crcr] {%
  3.8	0	0.3\\
  3.8	0	0\\
};
\addplot3 [densely dotted,color=mycolor2, line width=\lwA, line cap=round]
table[row sep=crcr] {%
  6.2	0	0.3\\
  6.2	0	0\\
};

\addplot3 [densely dotted,color=mycolor2, line width=\lwA, line cap=round]
table[row sep=crcr] {%
  3.8	0	0.3\\
  3	0	0.3\\
};
\addplot3 [densely dotted,color=mycolor2, line width=\lwA, line cap=round]
table[row sep=crcr] {%
  3.8	0	1.7\\
  3	0	1.7\\
};

%horizontal lines to image array
\addplot3 [densely dotted,color=mycolor2, line width=\lwA, line cap=round]%,opacity=0.2]
table[row sep=crcr] {%
  6.2	0	0.3\\
  9.8	0	0.3\\
};
\addplot3 [densely dotted,color=mycolor2, line width=\lwA, line cap=round]%,opacity=0.2]
table[row sep=crcr] {%
  6.2	0	1.7\\
  9.8	0	1.7\\
};




\addplot3 [color=mycolor3, densely dotted]
 table[row sep=crcr] {%
5	8	0\\
5	8	1\\
};
\addplot3 [color=mycolor3, only marks, mark=*, mark options={mark size=0.2pt,solid}]
table[row sep=crcr] {%
  5	8	0\\
};

\addplot3 [color=mycolor3, line width=0.5pt, only marks, mark=o, mark options={mark size=1.5pt,solid}]
 table[row sep=crcr] {%
5	8	1\\
};

\coordinate (wallA) at (axis cs:8,0,1);
\coordinate (wallB) at (axis cs:8,9,1);

\coordinate (va) at (axis cs:11,0,1);
\coordinate (vaR) at (axis cs:9.8,0,1);
\coordinate (vaL) at (axis cs:12.2,0,1);

\coordinate (pa) at (axis cs:5,0,1);
\coordinate (paL) at (axis cs:3.8,0,1);
\coordinate (paR) at (axis cs:6.2,0,1);

\coordinate (ue) at (axis cs:5,8,1);

%\draw[-,dotted] (va) -- (ue);
\draw[-,red,dotted] (vaL) -- (ue);
\draw[-,dotted] (vaR) -- (ue);


%\draw[dotted,red] (wallA) -- (wallB);

\coordinate (refl) at (intersection of wallA--wallB and va--ue);
\coordinate (reflL) at (intersection of wallA--wallB and vaL--ue);
\coordinate (reflR) at (intersection of wallA--wallB and vaR--ue);

\draw[<-,shorten <=0.5mm] (pa) -- (refl) -- (ue);

\draw[-,dotted] (pa) -- (refl) -- (ue);
\draw[-,dotted] (va) -- (refl);

\draw[<-,shorten <=0.5mm,red!50!white,densely dashed] (paL) -- (reflL) -- (ue);
\draw[<-,shorten <=0.5mm] (paR) -- (reflR) -- (ue);

%markes indictaing reflection points: circle...first(black) path, square...second(gray) path
%\draw plot[mark=o,mark options={mark size=1.5pt,color=black},only marks] coordinates {(refl) (pa) (va)};% (pa) (paR)};
%\draw plot[mark=o,mark options={mark size=1.5pt,color=black},only marks] coordinates {(paR) (vaR) (reflR)};% (pa) (paR)};
%\draw plot[mark=x,mark options={mark size=2.125pt,color=red!50!white},only marks] coordinates {(reflL) (paL) (vaL)};

\draw plot[mark=o,mark options={mark size=1.5pt,color=black},only marks] coordinates {(refl)};
\draw plot[mark=o,mark options={mark size=1.5pt,color=black},only marks] coordinates {(reflR)};
\draw plot[mark=x,mark options={mark size=2.125pt,color=red!50!white},only marks] coordinates {(reflL)};
\draw plot[mark=*,mark options={mark size=1pt,color=blue},only marks] coordinates {(paL) (paR) (pa)};
\draw plot[mark=*,mark options={mark size=1pt,color=blue,opacity=\wallopac},only marks] coordinates {(vaL) (vaR) (va)};

\node[blue,anchor=north,font={\footnotesize}] at (pa) {$\vm{a}$};
\node[blue,anchor=north,xshift=0.25mm,font={\footnotesize},text opacity=\vaannopac] at (va) {$\vm{a}_k$};
\node[anchor=west,font={\footnotesize}] at (ue) {$\vm{p}$};

\node[anchor=south west,font={\scriptsize}, inner sep=0mm,xshift=0mm,yshift=1mm,color=mycolor2text] at (paL) {$\vm{a}^{(m)}$};
\node[anchor=south west,font={\scriptsize}, inner sep=0mm,xshift=-1.25mm,yshift=1mm,color=mycolor2text] at (paR) {$\vm{a}^{(m')}$};

\node[anchor=west,font={\scriptsize}, inner sep=0mm,xshift=0.75mm,yshift=0.25mm,color=mycolor2text,text opacity=\vaannopac] at (vaR) {$\vm{a}_k^{(m')}$};
\node[anchor=east,font={\scriptsize}, inner sep=0mm,yshift=0.25mm,color=mycolor2text,text opacity=\vaannopac] at (vaL) {$\vm{a}_k^{(m)}$};

\coordinate (possible) at (axis cs:10.5,4.5,0);
\coordinate (impossible) at (axis cs:10.5,4.5,0.7);
%\node[black,anchor=east,font={\scriptsize},inner sep=0.1pt,text opacity=\annopac,rotate=\textangle] at (possible) {vis. refl. $v^\text{vis}_{k,m'}\rmv=\rmv1$};
%\node[red!80!white,anchor=east,font={\scriptsize},inner sep=0.1pt,text opacity=\annopac,rotate=\textangle] at (impossible) {invis. refl. $v^\text{vis}_{k,m}\rmv=\rmv0$};

%\draw[black,shorten >=1mm, shorten <=0.25mm,opacity=\annopac] (possible) -- (refl);
%\draw[black,shorten >=1mm, shorten <=0.25mm,opacity=\annopac] (possible) -- (reflR);
%\draw[red!50!white,shorten >=1mm, shorten <=0.25mm,opacity=\annopac] (impossible) -- (reflL);



%\draw[densely dotted] (refl) -- ++(0,0,1);



\end{axis}
\end{tikzpicture}%

==> tables/corridor_component_comparison_4x4_500MHz_floor.tex <==
%!TEX root = ../2023_EUCNC.tex
%$(4\times 4)$, 500~MHz, corridor
%\footnotesize
\scriptsize
\begin{tabular}{|l|r|r|r|r|r|}\hline
                  & L1                & L2 & L3 & L4 & L5 \\\hline
component         & \multicolumn{5}{c|}{component energy in \% of received signal energy (as mean $\pm$ std.dev.)} \\\hline\hline
strongest         & 42.4 $\pm$ 11.5  & 26.4 $\pm$  9.0 & 12.7 $\pm$  7.0  & 25.6 $\pm$  6.5  &  9.3 $\pm$  3.8  \\
2nd strongest     & 24.0 $\pm$  7.9  & 12.3 $\pm$  4.9 &  6.4 $\pm$  2.5  & 17.2 $\pm$  4.2  &  5.5 $\pm$  2.1  \\
3rd               &  8.5 $\pm$  3.8  &  7.7 $\pm$  3.0 &  4.3 $\pm$  1.6  & 11.8 $\pm$  3.5  &  3.6 $\pm$  1.2  \\
4th               &  4.5 $\pm$  2.4  &  4.8 $\pm$  1.7 &  3.3 $\pm$  1.3  &  7.2 $\pm$  3.6  &  2.6 $\pm$  0.8  \\
5th               &  2.2 $\pm$  1.2  &  3.4 $\pm$  1.6 &  2.6 $\pm$  0.9  &  3.6 $\pm$  1.7  &  2.0 $\pm$  0.6  \\
6th               &  1.3 $\pm$  0.7  &  2.3 $\pm$  1.0 &  2.0 $\pm$  0.7  &  2.3 $\pm$  1.1  &  1.7 $\pm$  0.5  \\\hline
$\sum$ over 20    & 87.0 $\pm$  3.6  & 63.1 $\pm$  7.1 & 38.4 $\pm$  8.9  & 69.7 $\pm$  6.3  & 31.8 $\pm$  6.7  \\
residual          & 12.3 $\pm$  3.4  & 35.3 $\pm$  6.8 & 60.9 $\pm$ 15.3  & 29.0 $\pm$  6.1  & 65.4 $\pm$  6.5  \\\hline\hline
%& \multicolumn{6}{c|}{SNR in dB (as mean $\pm$ std.dev.)} \\\hline
%strongest         & 17.31 $\pm$  1.78  & 10.53 $\pm$  2.06 &  4.75 $\pm$  2.54  &  11.38 $\pm$  1.46 &  3.10 $\pm$  2.27  &   \\
%2nd strongest     & 14.75 $\pm$  1.52  &  7.17 $\pm$  2.10 &  2.03 $\pm$  1.96  &   9.66 $\pm$  1.65 &  0.91 $\pm$  2.01  &   \\
%3rd               & 10.03 $\pm$  2.04  &  5.15 $\pm$  1.97 &  0.31 $\pm$  1.95  &   7.97 $\pm$  1.87 & -0.88 $\pm$  1.76  &   \\
%4th               &  7.10 $\pm$  2.29  &  3.10 $\pm$  1.70 & -0.86 $\pm$  1.96  &   5.44 $\pm$  2.92 & -2.21 $\pm$  1.76  &   \\
%5th               &  4.14 $\pm$  2.09  &  1.56 $\pm$  1.88 & -1.90 $\pm$  1.90  &   2.61 $\pm$  2.40 & -3.34 $\pm$  1.71  &   \\
%6th               &  2.08 $\pm$  1.90  & -0.09 $\pm$  2.01 & -2.94 $\pm$  1.83  &   0.63 $\pm$  2.28 & -4.09 $\pm$  1.68  &   \\\hline
%$\sum$ over 20    & 20.58 $\pm$  1.40  & 14.53 $\pm$  1.38 &  9.98 $\pm$  1.48  &  15.84 $\pm$  1.37 &  8.74 $\pm$  1.39  &   \\
%residual          & 11.95 $\pm$  0.00  & 11.95 $\pm$  0.00 & 12.00 $\pm$  0.46  &  11.95 $\pm$  0.00 & 11.95 $\pm$  0.00  &   \\
%signal            & 21.19 $\pm$  1.22  & 16.55 $\pm$  0.89 & 14.24 $\pm$  0.59  &  17.42 $\pm$  0.98 & 13.81 $\pm$  0.45  &   \\\hline\hline
%                  & \multicolumn{6}{c|}{component energy in \% of received signal energy (as mean $\pm$ std.dev.)} \\\hline
%direct path (1)   & 33.48 $\pm$ 18.96  &  8.51 $\pm$  4.51  &  5.29 $\pm$  8.02  & 18.89 $\pm$  6.64  &   NaN $\pm$   NaN  &   \\
%window north (2)  &  8.02 $\pm$  3.73  &  1.06 $\pm$  0.00  &  1.17 $\pm$  0.00  &  1.44 $\pm$  1.04  &  1.72 $\pm$  0.85  &   \\
%window south (3)  &  0.99 $\pm$  0.56  &  3.34 $\pm$  1.56  &  1.87 $\pm$  1.29  & 10.87 $\pm$  6.30  &  0.51 $\pm$  0.18  &   \\
%wall south (4)    & 28.96 $\pm$ 18.86  &  2.29 $\pm$  1.10  & 10.15 $\pm$  6.47  & 11.76 $\pm$  3.72  &  0.79 $\pm$  0.29  &   \\
%wall north (5)    & 19.57 $\pm$ 10.79  &  6.90 $\pm$  2.55  &  0.41 $\pm$  0.19  & 14.33 $\pm$  5.29  &   NaN $\pm$   NaN  &   \\
%wall n-s (6)      & 24.19 $\pm$ 11.32  &  2.33 $\pm$  1.04  &  3.33 $\pm$  2.80  &  8.85 $\pm$  4.26  &  3.20 $\pm$  1.62  &   \\\hline
%wall s-n (7)      &  6.04 $\pm$  3.48  &  6.61 $\pm$  6.96  &  5.29 $\pm$  3.33  & 15.30 $\pm$  6.61  &  0.82 $\pm$  0.15  & x  \\
%floor (8)         &  0.56 $\pm$  0.00  &   NaN $\pm$   NaN  &   NaN $\pm$   NaN  &   NaN $\pm$   NaN  &   NaN $\pm$   NaN  & x  \\
%floor-s (9)       &  1.22 $\pm$  0.20  &  0.42 $\pm$  0.00  &   NaN $\pm$   NaN  &   NaN $\pm$   NaN  &   NaN $\pm$   NaN  & x  \\
%floor-n (10)      &   NaN $\pm$   NaN  & 36.33 $\pm$  0.00  &   NaN $\pm$   NaN  &   NaN $\pm$   NaN  &   NaN $\pm$   NaN  & x  \\\hline
%$\sum$ over 10    & 41.49 $\pm$ 12.67  &  2.62 $\pm$  3.04  &  0.00 $\pm$  0.00  &  0.00 $\pm$  0.00  &  0.98 $\pm$  0.61  &   \\\hline%\hline
\end{tabular}
 


==> tables/corridor_component_comparison_4x4_500MHz_round.tex <==
%!TEX root = ../2023_EUCNC.tex
%$(4\times 4)$, 500~MHz, corridor
%\footnotesize
\scriptsize
\begin{tabular}{|l|r|r|r|r|r|r|}\hline
                  & L1                & L2 & L3 & L4 & L5 & L8 \\\hline
component   & \multicolumn{6}{c|}{component energy in \% of received signal energy (as mean $\pm$ std.dev.)} \\\hline\hline
strongest         & 42.48 $\pm$ 11.59  & 26.47 $\pm$  9.04 & 12.78 $\pm$  7.05  & 25.61 $\pm$  6.52  &  9.32 $\pm$  3.88  &   \\
2nd strongest     & 24.03 $\pm$  7.94  & 12.37 $\pm$  4.92 &  6.43 $\pm$  2.50  & 17.26 $\pm$  4.22  &  5.54 $\pm$  2.16  &   \\
3rd               &  8.52 $\pm$  3.86  &  7.76 $\pm$  3.02 &  4.35 $\pm$  1.68  & 11.87 $\pm$  3.59  &  3.60 $\pm$  1.27  &   \\
4th               &  4.50 $\pm$  2.48  &  4.82 $\pm$  1.79 &  3.34 $\pm$  1.32  &  7.22 $\pm$  3.62  &  2.64 $\pm$  0.89  &   \\
5th               &  2.25 $\pm$  1.20  &  3.47 $\pm$  1.60 &  2.61 $\pm$  0.96  &  3.65 $\pm$  1.72  &  2.03 $\pm$  0.69  &   \\
6th               &  1.39 $\pm$  0.77  &  2.38 $\pm$  1.09 &  2.04 $\pm$  0.74  &  2.31 $\pm$  1.13  &  1.70 $\pm$  0.53  &   \\\hline
$\sum$ over 20    & 87.08 $\pm$  3.63  & 63.17 $\pm$  7.11 & 38.47 $\pm$  8.90  & 69.71 $\pm$  6.37  & 31.81 $\pm$  6.79  &   \\
residual          & 12.38 $\pm$  3.48  & 35.33 $\pm$  6.83 & 60.90 $\pm$ 15.32  & 29.04 $\pm$  6.11  & 65.46 $\pm$  6.54  &   \\\hline\hline
%& \multicolumn{6}{c|}{SNR in dB (as mean $\pm$ std.dev.)} \\\hline
%strongest         & 17.31 $\pm$  1.78  & 10.53 $\pm$  2.06 &  4.75 $\pm$  2.54  &  11.38 $\pm$  1.46 &  3.10 $\pm$  2.27  &   \\
%2nd strongest     & 14.75 $\pm$  1.52  &  7.17 $\pm$  2.10 &  2.03 $\pm$  1.96  &   9.66 $\pm$  1.65 &  0.91 $\pm$  2.01  &   \\
%3rd               & 10.03 $\pm$  2.04  &  5.15 $\pm$  1.97 &  0.31 $\pm$  1.95  &   7.97 $\pm$  1.87 & -0.88 $\pm$  1.76  &   \\
%4th               &  7.10 $\pm$  2.29  &  3.10 $\pm$  1.70 & -0.86 $\pm$  1.96  &   5.44 $\pm$  2.92 & -2.21 $\pm$  1.76  &   \\
%5th               &  4.14 $\pm$  2.09  &  1.56 $\pm$  1.88 & -1.90 $\pm$  1.90  &   2.61 $\pm$  2.40 & -3.34 $\pm$  1.71  &   \\
%6th               &  2.08 $\pm$  1.90  & -0.09 $\pm$  2.01 & -2.94 $\pm$  1.83  &   0.63 $\pm$  2.28 & -4.09 $\pm$  1.68  &   \\\hline
%$\sum$ over 20    & 20.58 $\pm$  1.40  & 14.53 $\pm$  1.38 &  9.98 $\pm$  1.48  &  15.84 $\pm$  1.37 &  8.74 $\pm$  1.39  &   \\
%residual          & 11.95 $\pm$  0.00  & 11.95 $\pm$  0.00 & 12.00 $\pm$  0.46  &  11.95 $\pm$  0.00 & 11.95 $\pm$  0.00  &   \\
%signal            & 21.19 $\pm$  1.22  & 16.55 $\pm$  0.89 & 14.24 $\pm$  0.59  &  17.42 $\pm$  0.98 & 13.81 $\pm$  0.45  &   \\\hline\hline
%                  & \multicolumn{6}{c|}{component energy in \% of received signal energy (as mean $\pm$ std.dev.)} \\\hline
%direct path (1)   & 33.48 $\pm$ 18.96  &  8.51 $\pm$  4.51  &  5.29 $\pm$  8.02  & 18.89 $\pm$  6.64  &   NaN $\pm$   NaN  &   \\
%window north (2)  &  8.02 $\pm$  3.73  &  1.06 $\pm$  0.00  &  1.17 $\pm$  0.00  &  1.44 $\pm$  1.04  &  1.72 $\pm$  0.85  &   \\
%window south (3)  &  0.99 $\pm$  0.56  &  3.34 $\pm$  1.56  &  1.87 $\pm$  1.29  & 10.87 $\pm$  6.30  &  0.51 $\pm$  0.18  &   \\
%wall south (4)    & 28.96 $\pm$ 18.86  &  2.29 $\pm$  1.10  & 10.15 $\pm$  6.47  & 11.76 $\pm$  3.72  &  0.79 $\pm$  0.29  &   \\
%wall north (5)    & 19.57 $\pm$ 10.79  &  6.90 $\pm$  2.55  &  0.41 $\pm$  0.19  & 14.33 $\pm$  5.29  &   NaN $\pm$   NaN  &   \\
%wall n-s (6)      & 24.19 $\pm$ 11.32  &  2.33 $\pm$  1.04  &  3.33 $\pm$  2.80  &  8.85 $\pm$  4.26  &  3.20 $\pm$  1.62  &   \\\hline
%wall s-n (7)      &  6.04 $\pm$  3.48  &  6.61 $\pm$  6.96  &  5.29 $\pm$  3.33  & 15.30 $\pm$  6.61  &  0.82 $\pm$  0.15  & x  \\
%floor (8)         &  0.56 $\pm$  0.00  &   NaN $\pm$   NaN  &   NaN $\pm$   NaN  &   NaN $\pm$   NaN  &   NaN $\pm$   NaN  & x  \\
%floor-s (9)       &  1.22 $\pm$  0.20  &  0.42 $\pm$  0.00  &   NaN $\pm$   NaN  &   NaN $\pm$   NaN  &   NaN $\pm$   NaN  & x  \\
%floor-n (10)      &   NaN $\pm$   NaN  & 36.33 $\pm$  0.00  &   NaN $\pm$   NaN  &   NaN $\pm$   NaN  &   NaN $\pm$   NaN  & x  \\\hline
%$\sum$ over 10    & 41.49 $\pm$ 12.67  &  2.62 $\pm$  3.04  &  0.00 $\pm$  0.00  &  0.00 $\pm$  0.00  &  0.98 $\pm$  0.61  &   \\\hline%\hline
\end{tabular}
 


==> tables/demoroom_component_comparison_4x4_500MHz_floor.tex <==
%!TEX root = ../2023_EUCNC.tex
%$(4\times 4)$, 500~MHz
%\footnotesize
\scriptsize
\begin{tabular}{|l|r|r|r|r|r|r|}\hline
                  & M1                & M2 & M3 & M4 & M5 & M6 \\\hline
component         & \multicolumn{6}{c|}{component energy in \% of received signal energy (as mean $\pm$ std.dev.)} \\\hline\hline
strongest         & 85.8 $\pm$  6.5 & 76.5 $\pm$ 15.3 & 67.2 $\pm$  9.4 & 43.3 $\pm$ 14.6 & 85.4 $\pm$ 17.5 & 65.2 $\pm$  9.1 \\
2nd strongest     &  3.9 $\pm$  1.9 &  4.7 $\pm$  4.6 &  9.7 $\pm$  5.4 & 16.1 $\pm$  8.2 &  6.7 $\pm$  9.5 & 14.9 $\pm$  8.1 \\
3rd               &  2.1 $\pm$  1.3 &  1.4 $\pm$  1.3 &  3.9 $\pm$  2.3 &  6.7 $\pm$  4.1 &  1.2 $\pm$  1.5 &  6.1 $\pm$  3.6 \\
4th               &  1.1 $\pm$  0.6 &  0.7 $\pm$  0.7 &  2.4 $\pm$  1.0 &  4.2 $\pm$  1.9 &  0.6 $\pm$  0.6 &  2.8 $\pm$  1.5 \\
5th               &  0.8 $\pm$  0.3 &  0.5 $\pm$  0.4 &  1.8 $\pm$  0.7 &  3.1 $\pm$  1.3 &  0.4 $\pm$  0.4 &  1.8 $\pm$  0.8 \\
6th               &  0.6 $\pm$  0.3 &  0.4 $\pm$  0.3 &  1.3 $\pm$  0.5 &  2.4 $\pm$  0.9 &  0.3 $\pm$  0.3 &  1.3 $\pm$  0.4 \\\hline
$\sum$ over 20    & \textbf{96.5} $\pm$  1.1 & \textbf{97.8} $\pm$  1.6 & 91.1 $\pm$  2.8 & 82.3 $\pm$  4.7 & \textbf{97.8} $\pm$  1.7 & 94.1 $\pm$  1.6 \\
residual          &  3.1 $\pm$  1.0 &  1.9 $\pm$  1.4 &  7.9 $\pm$  2.6 & 15.9 $\pm$  4.2 &  1.9 $\pm$  1.5 &  5.3 $\pm$  1.4 \\\hline\hline
% & \multicolumn{6}{c|}{SNR in dB (as mean $\pm$ std.dev.)} \\\hline
%strongest         & 26.35 $\pm$  1.58 & 28.89 $\pm$  3.60 & 21.26 $\pm$  1.84 & 16.06 $\pm$  2.37 & 29.70 $\pm$  4.31 & 22.80 $\pm$  1.55 \\
%2nd strongest     & 12.51 $\pm$  2.78 & 14.89 $\pm$  3.74 & 12.17 $\pm$  2.92 & 11.32 $\pm$  3.00 & 16.09 $\pm$  5.21 & 15.82 $\pm$  2.25 \\
%3rd               &  9.73 $\pm$  2.83 & 10.30 $\pm$  2.48 &  8.38 $\pm$  2.14 &  7.61 $\pm$  2.30 &  9.40 $\pm$  2.81 & 11.87 $\pm$  2.69 \\
%4th               &  7.23 $\pm$  2.20 &  7.58 $\pm$  2.42 &  6.50 $\pm$  1.71 &  5.82 $\pm$  1.92 &  7.20 $\pm$  2.42 &  8.77 $\pm$  2.28 \\
%5th               &  5.60 $\pm$  1.83 &  5.87 $\pm$  2.08 &  5.28 $\pm$  1.60 &  4.59 $\pm$  1.73 &  5.54 $\pm$  1.89 &  6.99 $\pm$  1.89 \\
%6th               &  4.46 $\pm$  1.69 &  4.63 $\pm$  1.78 &  4.12 $\pm$  1.54 &  3.53 $\pm$  1.66 &  4.39 $\pm$  1.60 &  5.58 $\pm$  1.56 \\\hline
%$\sum$ over 20    & 26.87 $\pm$  1.37 & 30.06 $\pm$  3.21 & 22.62 $\pm$  1.56 & 19.09 $\pm$  1.43 & 30.39 $\pm$  3.97 & 24.43 $\pm$  1.21 \\
%residual          & 11.81 $\pm$  0.00 & 11.81 $\pm$  0.00 & 11.81 $\pm$  0.00 & 11.82 $\pm$  0.00 & 11.81 $\pm$  0.00 & 11.81 $\pm$  0.00 \\
%signal            & 27.02 $\pm$  1.32 & 30.15 $\pm$  3.14 & 23.03 $\pm$  1.42 & 19.94 $\pm$  1.18 & 30.48 $\pm$  3.90 & 24.70 $\pm$  1.13 \\\hline\hline
% & \multicolumn{6}{c|}{component energy in \% of received signal energy (as mean $\pm$ std.dev.)} \\\hline
%\textrm{direct path} (1)      & 85.86 $\pm$  6.50 & 76.28 $\pm$ 16.26 & 66.87 $\pm$ 10.67 & 36.61 $\pm$ 17.72 & 38.66 $\pm$ 41.41 & 61.01 $\pm$ 19.31 \\
%window (2)                    &  1.94 $\pm$  1.71 &  0.41 $\pm$  0.68 &  2.91 $\pm$  3.38 &  2.03 $\pm$  2.38 &  0.32 $\pm$  0.54 &  6.76 $\pm$  5.06 \\
%\textit{window-doorwall} (3)  &  0.63 $\pm$  0.60 &  0.54 $\pm$  1.10 &  0.56 $\pm$  0.30 &  1.20 $\pm$  0.80 &  0.36 $\pm$  0.55 &  1.19 $\pm$  0.83 \\
%\textit{window-whiteboard} (4)&  0.31 $\pm$  0.23 &  0.08 $\pm$  0.04 &  0.60 $\pm$  0.30 &  0.59 $\pm$  0.11 &                   &  0.26 $\pm$  0.14 \\
%whiteboard (5)                &  0.51 $\pm$  0.47 &  0.22 $\pm$  0.19 &  1.48 $\pm$  0.96 &  3.99 $\pm$  2.84 &  0.14 $\pm$  0.12 &  0.37 $\pm$  0.18 \\
%floor (6)                     &  1.04 $\pm$  1.01 &  0.81 $\pm$  0.92 &  1.83 $\pm$  1.12 &  0.92 $\pm$  0.77 &  0.13 $\pm$  0.18 &  1.79 $\pm$  1.66 \\
%ceiling (7)                   &  0.23 $\pm$  0.15 &  0.07 $\pm$  0.07 &  2.29 $\pm$  2.24 &  0.63 $\pm$  0.25 &  0.10 $\pm$  0.08 &  0.59 $\pm$  0.42 \\
%doorwall (8)                  &  2.52 $\pm$  2.15 &  1.18 $\pm$  1.85 &  8.23 $\pm$  6.13 & 11.98 $\pm$ 13.99 &  0.94 $\pm$  2.48 &  9.50 $\pm$  9.13 \\\hline
%$\sum$ over 8                 & \textbf{91.00} $\pm$  6.29 & 77.81 $\pm$ 16.82 & \textbf{81.21} $\pm$  6.72 & 23.92 $\pm$ 10.27 & \textbf{84.38} $\pm$ 18.73 & 82.15 $\pm$  6.02 \\\hline%\hline
\end{tabular}
 


==> tables/demoroom_component_comparison_4x4_500MHz_round.tex <==
%!TEX root = ../2023_EUCNC.tex
%$(4\times 4)$, 500~MHz
%\footnotesize
\scriptsize
\begin{tabular}{|l|r|r|r|r|r|r|}\hline
                  & M1                & M2 & M3 & M4 & M5 & M6 \\\hline
component   & \multicolumn{6}{c|}{component energy in \% of received signal energy (as mean $\pm$ std.dev.)} \\\hline\hline
strongest         & 85.86 $\pm$  6.50 & 76.56 $\pm$ 15.39 & 67.28 $\pm$  9.40 & 43.32 $\pm$ 14.65 & 85.41 $\pm$ 17.52 & 65.28 $\pm$  9.10 \\
2nd strongest     &  3.95 $\pm$  1.99 &  4.76 $\pm$  4.67 &  9.73 $\pm$  5.48 & 16.12 $\pm$  8.27 &  6.75 $\pm$  9.53 & 14.98 $\pm$  8.12 \\
3rd               &  2.18 $\pm$  1.35 &  1.42 $\pm$  1.37 &  3.95 $\pm$  2.36 &  6.77 $\pm$  4.17 &  1.22 $\pm$  1.56 &  6.12 $\pm$  3.64 \\
4th               &  1.19 $\pm$  0.64 &  0.79 $\pm$  0.71 &  2.43 $\pm$  1.07 &  4.26 $\pm$  1.95 &  0.69 $\pm$  0.64 &  2.88 $\pm$  1.56 \\
5th               &  0.80 $\pm$  0.38 &  0.54 $\pm$  0.45 &  1.82 $\pm$  0.74 &  3.17 $\pm$  1.35 &  0.46 $\pm$  0.43 &  1.84 $\pm$  0.82 \\
6th               &  0.62 $\pm$  0.30 &  0.40 $\pm$  0.34 &  1.38 $\pm$  0.55 &  2.46 $\pm$  0.98 &  0.35 $\pm$  0.32 &  1.30 $\pm$  0.46 \\\hline
$\sum$ over 20    & \textbf{96.51} $\pm$  1.17 & \textbf{97.89} $\pm$  1.61 & 91.19 $\pm$  2.87 & 82.36 $\pm$  4.70 & \textbf{97.84} $\pm$  1.76 & 94.11 $\pm$  1.61 \\
residual          &  3.16 $\pm$  1.06 &  1.91 $\pm$  1.46 &  7.98 $\pm$  2.60 & 15.98 $\pm$  4.25 &  1.95 $\pm$  1.59 &  5.33 $\pm$  1.45 \\\hline\hline
% & \multicolumn{6}{c|}{SNR in dB (as mean $\pm$ std.dev.)} \\\hline
%strongest         & 26.35 $\pm$  1.58 & 28.89 $\pm$  3.60 & 21.26 $\pm$  1.84 & 16.06 $\pm$  2.37 & 29.70 $\pm$  4.31 & 22.80 $\pm$  1.55 \\
%2nd strongest     & 12.51 $\pm$  2.78 & 14.89 $\pm$  3.74 & 12.17 $\pm$  2.92 & 11.32 $\pm$  3.00 & 16.09 $\pm$  5.21 & 15.82 $\pm$  2.25 \\
%3rd               &  9.73 $\pm$  2.83 & 10.30 $\pm$  2.48 &  8.38 $\pm$  2.14 &  7.61 $\pm$  2.30 &  9.40 $\pm$  2.81 & 11.87 $\pm$  2.69 \\
%4th               &  7.23 $\pm$  2.20 &  7.58 $\pm$  2.42 &  6.50 $\pm$  1.71 &  5.82 $\pm$  1.92 &  7.20 $\pm$  2.42 &  8.77 $\pm$  2.28 \\
%5th               &  5.60 $\pm$  1.83 &  5.87 $\pm$  2.08 &  5.28 $\pm$  1.60 &  4.59 $\pm$  1.73 &  5.54 $\pm$  1.89 &  6.99 $\pm$  1.89 \\
%6th               &  4.46 $\pm$  1.69 &  4.63 $\pm$  1.78 &  4.12 $\pm$  1.54 &  3.53 $\pm$  1.66 &  4.39 $\pm$  1.60 &  5.58 $\pm$  1.56 \\\hline
%$\sum$ over 20    & 26.87 $\pm$  1.37 & 30.06 $\pm$  3.21 & 22.62 $\pm$  1.56 & 19.09 $\pm$  1.43 & 30.39 $\pm$  3.97 & 24.43 $\pm$  1.21 \\
%residual          & 11.81 $\pm$  0.00 & 11.81 $\pm$  0.00 & 11.81 $\pm$  0.00 & 11.82 $\pm$  0.00 & 11.81 $\pm$  0.00 & 11.81 $\pm$  0.00 \\
%signal            & 27.02 $\pm$  1.32 & 30.15 $\pm$  3.14 & 23.03 $\pm$  1.42 & 19.94 $\pm$  1.18 & 30.48 $\pm$  3.90 & 24.70 $\pm$  1.13 \\\hline\hline
% & \multicolumn{6}{c|}{component energy in \% of received signal energy (as mean $\pm$ std.dev.)} \\\hline
%\textrm{direct path} (1)      & 85.86 $\pm$  6.50 & 76.28 $\pm$ 16.26 & 66.87 $\pm$ 10.67 & 36.61 $\pm$ 17.72 & 38.66 $\pm$ 41.41 & 61.01 $\pm$ 19.31 \\
%window (2)                    &  1.94 $\pm$  1.71 &  0.41 $\pm$  0.68 &  2.91 $\pm$  3.38 &  2.03 $\pm$  2.38 &  0.32 $\pm$  0.54 &  6.76 $\pm$  5.06 \\
%\textit{window-doorwall} (3)  &  0.63 $\pm$  0.60 &  0.54 $\pm$  1.10 &  0.56 $\pm$  0.30 &  1.20 $\pm$  0.80 &  0.36 $\pm$  0.55 &  1.19 $\pm$  0.83 \\
%\textit{window-whiteboard} (4)&  0.31 $\pm$  0.23 &  0.08 $\pm$  0.04 &  0.60 $\pm$  0.30 &  0.59 $\pm$  0.11 &                   &  0.26 $\pm$  0.14 \\
%whiteboard (5)                &  0.51 $\pm$  0.47 &  0.22 $\pm$  0.19 &  1.48 $\pm$  0.96 &  3.99 $\pm$  2.84 &  0.14 $\pm$  0.12 &  0.37 $\pm$  0.18 \\
%floor (6)                     &  1.04 $\pm$  1.01 &  0.81 $\pm$  0.92 &  1.83 $\pm$  1.12 &  0.92 $\pm$  0.77 &  0.13 $\pm$  0.18 &  1.79 $\pm$  1.66 \\
%ceiling (7)                   &  0.23 $\pm$  0.15 &  0.07 $\pm$  0.07 &  2.29 $\pm$  2.24 &  0.63 $\pm$  0.25 &  0.10 $\pm$  0.08 &  0.59 $\pm$  0.42 \\
%doorwall (8)                  &  2.52 $\pm$  2.15 &  1.18 $\pm$  1.85 &  8.23 $\pm$  6.13 & 11.98 $\pm$ 13.99 &  0.94 $\pm$  2.48 &  9.50 $\pm$  9.13 \\\hline
%$\sum$ over 8                 & \textbf{91.00} $\pm$  6.29 & 77.81 $\pm$ 16.82 & \textbf{81.21} $\pm$  6.72 & 23.92 $\pm$ 10.27 & \textbf{84.38} $\pm$ 18.73 & 82.15 $\pm$  6.02 \\\hline%\hline
\end{tabular}
 

